Theoretically Efficient Parallel Graph Algorithms Can Be Fast and Scalable

There has been significant recent interest in parallel graph processing due to the need to quickly analyze the large graphs available today. Many graph codes have been designed for distributed memory or external memory. However, today even the largest publicly-available real-world graph (the Hyperlink Web graph with over 3.5 billion vertices and 128 billion edges) can fit in the memory of a single commodity multicore server. Nevertheless, most experimental work in the literature report results on much smaller graphs, and the ones for the Hyperlink graph use distributed or external memory. Therefore, it is natural to ask whether we can efficiently solve a broad class of graph problems on this graph in memory. This paper shows that theoretically-efficient parallel graph algorithms can scale to the largest publicly-available graphs using a single machine with a terabyte of RAM, processing them in minutes. We give implementations of theoretically-efficient parallel algorithms for 20 important graph problems. We also present the optimizations and techniques that we used in our implementations, which were crucial in enabling us to process these large graphs quickly. We show that the running times of our implementations outperform existing state-of-the-art implementations on the largest real-world graphs. For many of the problems that we consider, this is the first time they have been solved on graphs at this scale. We have made the implementations developed in this work publicly-available as the Graph-Based Benchmark Suite (GBBS).

==> inputs/additional-techniques.tex <==
\section{Additional Techniques}\label{sec:additionaltechniques}


==> inputs/benchmarks.tex <==
\section{Benchmarking Parallel Graph Algorithms}\label{sec:benchmarking}

%\myparagraph{Benchmarking Parallel Graph Algorithms}
There are a
surprising number of existing benchmarks of parallel graph algorithms.
SSCA~\cite{bader2005design}, an early graph processing benchmark,
specifies four graph kernels, which include generating graphs in
adjacency list format, subgraph extraction, and graph clustering. The
Problem Based Benchmark Suite (PBBS)~\cite{shun2012brief} is a general
benchmark of parallel algorithms that includes 6 problems on graphs
(breadth-first search (BFS), spanning forest, minimum spanning forest,
maximal independent set, maximal matching, and graph separators). The
PBBS benchmarks are problem-based in that they are defined only in
terms of the input and output without any specification of the
algorithm used to solve the problem.  We follow the style of PBBS in
this paper of defining the input and output requirements for each
problem. The Graph Algorithm Platform (GAP) Benchmark
Suite~\cite{BeamerAP15} specifies six kernels for BFS, SSSP,
PageRank, connectivity, betweenness centrality, and triangle counting.
%% Compared to our benchmark, GAP is more focused on benchmarking graph algorithm
%% performance and does not require that kernel implementations are theoretically
%% efficient. \julian{I don't think any of the benchmarks have this requirement.}

Several recent benchmarks characterize the architectural properties of
parallel graph algorithms. GraphBIG~\cite{nai2015graphbig} describes
12 applications, including several problems that we consider, like
$k$-core and graph coloring (using the Jones-Plassmann algorithm), but also problems like depth-first search,
which are difficult to parallelize, as well as dynamic graph
operations. CRONO~\cite{ahmad2015crono} implements 10 graph
algorithms, including all-pairs shortest paths, exact betweenness
centrality, traveling salesman, and depth-first
search. LDBC~\cite{iosup16ldbc} is an industry-driven benchmark that
selects six algorithms that are considered representative of graph
processing including BFS, and several algorithms based on label
propagation.

Unfortunately, all of the existing graph algorithm benchmarks we are aware of
restrict their evaluation to very small graphs, often on the order of tens
or hundreds of millions of edges, with the largest graphs in the benchmarks having
about two billion edges. As real-world graphs are frequently several orders of
magnitude larger than this, evaluation on such small graphs makes it hard to
judge whether the algorithms or results from a benchmark scale to
terabyte-scale graphs.



==> inputs/problems.tex <==
\section{Problems}\label{sec:problems}

Most problems we consider in this paper are defined so that their output is
unambiguous.  However, some problems like Graph Coloring and Approximate Set
Cover have many valid answers, with some answers, like a coloring where every
vertex is colored with a color corresponding to its own id, being trivial to
find. In these cases, the desired output is usually a solution produced using a
heuristic or approximation algorithms. For such problems, instead of expecting
a particular output, we make a restriction on the solution-quality of the
output. We give more details on this restriction in section todo and mark such
problems with a $\dagger$ superscript.

\myparagraph{Connectivity}\\
Input: $G=(V,E)$, an undirected graph\\
Output: $\mathcal{L}$, a mapping from each vertex to the label of its connected component.

\myparagraph{Biconnectivity}\\
Input: $G=(V,E)$, an undirected graph\\
Output: $\mathcal{L}$, a mapping from each edge the label of its biconnected component.

\myparagraph{SCC}\\
Input: $G(V, E)$, a directed graph\\
Output: $\mathcal{L}$, a mapping from each vertex to the label of its strongly-connected component.

\myparagraph{Low-Diameter Decomposition}\\
Input: $G=(V, E)$, a directed graph, $0 < \beta < 1$\\
Output: $\mathcal{L}$, a mapping from each vertex to a component s.t. the number of intercomponent edges is $O(\beta m$) and the diameter of each component is $O(\frac{\log n}{\beta})$.

\myparagraph{Maximal Independent Set}\\
Input: $G=(V, E)$, an undirected graph\\
Output: $U \subseteq V$, a set of vertices s.t. no vertices in $U$ are neighbors of each other and all vertices in $V \setminus U$ have a neighbor in $U$.

\myparagraph{Maximal Matching}\\
Input: $G=(V, E)$, an undirected graph\\
Output: $E' \subseteq E$, a set of edges s.t. no edges in $E'$ share endpoints and all edges in $E \setminus E'$ share an endpoint with some edge in $E'$.

\myparagraph{Graph Coloring}$^{\dagger}$\\
Input: $G=(V, E)$, an undirected graph\\
Output: $C$, a mapping from each vertex to a color s.t. for each edge $(u, v) \in E$, $C(u) \neq C(v)$.

\myparagraph{Single Source Betweenness Centrality}\\
Input: $G=(V, E)$, an undirected graph, $\src \in V$\\
Output: $S$, a mapping from each vertex $v$ to the centrality contribution from all $(\src, t)$ shortest paths that pass through $v$.

\myparagraph{SSSP (unweighted)}\\
Input: $G=(V, E)$, an unweighted graph, $\src \in V$\\
Output: $D$, a mapping where $D[v]$ is the shortest path distance from $\src$ to $v$ in $G$ and $\infty$ if $v$ is unreachable.

\myparagraph{SSSP (integral weights)}\\
Input: $G=(V, E, w)$, a weighted graph with integral edge weights, $\src \in V$\\
Output: $D$, a mapping where $D[v]$ is the shortest path distance from $\src$ to $v$ in $G$ and $\infty$ if $v$ is unreachable.

\myparagraph{SSSP (negative weights)}\\
Input: $G=(V, E, w)$, a weighted graph, $\src \in V$\\
Output: $D$, a mapping where $D[v]$ is the shortest path distance from $\src$ to $v$ in $G$ and $\infty$ if $v$ is unreachable. All distances must be $-\infty$ if $G$ contains a negative-weight cycle reachable from $\src$.

\myparagraph{Minimum Spanning Forest}\\
Input: $G=(V, E, w)$, a weighted graph\\
Output: $T$, a set of edges representing a minimum spanning forest of $G$.

\myparagraph{$k$-core}\\
Input: $G=(V, E)$, an undirected graph\\
Output: $D$, a mapping from each vertex to its coreness value.

\myparagraph{Approximate Set Cover}$^{\dagger}$\\
Input: $G=(V, E)$, an undirected graph representing a set-cover instance\\
Output: $S \subseteq V$, a set of sets s.t. $\cup_{s \in s} N(s) = V$.

\myparagraph{Triangle Counting}\\
Input: $G=(V, E)$, an undirected graph\\
Output: $T$, a mapping from each vertex to the number of triangles incident to it.


